The Computational Complexity of Circuit Discovery for Inner Interpretability

Many proposed applications of neural networks in machine learning, cognitive/brain science, and society hinge on the feasibility of inner interpretability via circuit discovery. This calls for empirical and theoretical explorations of viable algorithmic options. Despite advances in the design and testing of heuristics, there are concerns about their scalability and faithfulness at a time when we lack understanding of the complexity properties of the problems they are deployed to solve. To address this, we study circuit discovery with classical and parameterized computational complexity theory: (1) we describe a conceptual scaffolding to reason about circuit finding queries in terms of affordances for description, explanation, prediction and control; (2) we formalize a comprehensive set of queries for mechanistic explanation, and propose a formal framework for their analysis; (3) we use it to settle the complexity of many query variants and relaxations of practical interest on multi-layer perceptrons. Our findings reveal a challenging complexity landscape. Many queries are intractable, remain fixed-parameter intractable relative to model/circuit features, and inapproximable under additive, multiplicative, and probabilistic approximation schemes. To navigate this landscape, we prove there exist transformations to tackle some of these hard problems with better-understood heuristics, and prove the tractability or fixed-parameter tractability of more modest queries which retain useful affordances. This framework allows us to understand the scope and limits of interpretability queries, explore viable options, and compare their resource demands on existing and future architectures.

==> notes/membership.tex <==


%%%% NECESSARY CIRCUIT (LOCAL)

Let us first show membership in $\Sigma^p_2$. 
Using the alternating-quantifier definition of classes in the polynomial hierarchy, membership of a decision problem $\Pi$ in $\Sigma^p_2$ can be proved by showing that solving $\Pi$ for input $I$ is equivalent to solving a quantified formula of the form $\exists (x) \forall (y) : p(x, y)$ where both the sizes of $x$ and $y$ and the evaluation time of predicate formula $p()$ are upper-bounded by polynomials in $|I|$. 

Such a formula 

\[
\exists (N \subseteq M) \forall (N' \subseteq M \wedge 
                                 I \in \{0,1\}^{\#n_{in}})
            (\text{IsSuffCircuit}(N', M, I) \rightarrow N \cap N' \neq \emptyset)
\]




==> notes/notes_CMSNC.tex <==


\begin{definition}
An entity $x$ with property $P$ is {\em minimal} if there is no non-empty
subset of elements in $x$ that can be deleted to create an entity $x'$ with
property $P$.
\end{definition}

\noindent
{\sc Minimal local sufficient circuit} (MnlLSC) \\
{\em Input}: A multi-layer perceptron $M$ of depth $cd_g$ with $\#n_{tot,g}$ neurons
              and maximum layer width $cw_g$, connection-value matrices $W_1, W_2, \ldots, 
              W_{cd_g}$, neuron bias vector $B$, a Boolean input vector $I$ of length 
              $\#n_{g,in}$, and integers $d$ and $w$ such that $1 \leq d \leq 
              cd_g$ and $1 \leq w \leq cw_g$. \\
{\em Output}: A minimal subcircuit $C$ of $M$ of depth $cd_r \leq d$ 
               with maximum layer width $cw_r \leq w$ that produces the
               same output on input $I$ as $M$.

\vspace*{0.1in}

\noindent
{\sc Minimal global sufficient circuit} (MnlGSC) \\
{\em Input}: A multi-layer perceptron $M$ of depth $cd_g$ with $\#n_{tot,g}$ neurons
              and maximum layer width $cw_g$, connection-value matrices $W_1, W_2, \ldots, 
              W_{cd_g}$, neuron bias vector $B$, and integers $d$ and $w$
	      such that $1 \leq d \leq cd_g$ and $1 \leq w \leq cw_g$. \\
{\em Output}: A minimal subcircuit $C$ of $M$ of depth $cd_r \leq d$ with
               maximum layer width $cw_r \leq w$ that produces the
               same output as $M$ on every possible Boolean input vector of
               length $\#_{in,g}$.

\vspace*{0.1in}

\noindent
{\sc Minimal Local Necessary Circuit} (MnlLNC) \\
{\em Input}: A multi-layer perceptron $M$ of depth $cd$ with $\#n_{tot}$
              neurons and maximum layer width $cw$, connection-value 
              matrices $W_1, W_2, \ldots, W_{cd}$, neuron bias vector $B$,
              and a Boolean input vector $I$ of length $\#n_{in}$. \\
{\em Output}: A minimal subset $N'$ of the $|N|$ neurons
               in $M$ such that $N' \cap C \neq \emptyset$ for every 
	       sufficient circuit $C$ of $M$ relative to $I$?

\vspace*{0.1in}

\noindent
{\sc Minimal Global Necessary Circuit} (MnlGNC) \\
{\em Input}: A multi-layer perceptron $M$ of depth $cd$ with $\#n_{tot}$
              neurons and maximum layer width $cw$, connection-value 
              matrices $W_1, W_2, \ldots, W_{cd}$, and neuron bias vector 
	      $B$. \\
{\em Output}: A minimal subset $N'$ of the $|N|$ neurons
               in $M$ such that for for every possible Boolean input
	       vector $I$ of length $\#n_{in}$, $N' \cap C \neq \emptyset$
	       for every sufficient circuit $C$ of $M$ relative to $I$.

\vspace*{0.1in}

We will use previous results for the following problems 
to prove our results for the problems above.

\vspace*{0.1in}

\noindent
{\sc Minimal vertex cover} (MnlVC) \cite[Problem 4]{Val79Enum} \\
{\em Input}: An undirected graph $G = (V, E)$. \\
{\em Output}: A minimal vertex cover of $G$, i.e., 
               a minimal subset $V' \subseteq V$ such that for 
                 all $(u, v) \in E$, at least one of $u$ or $v$ is in $V'$. 

\vspace*{0.1in}

\noindent
{\sc Minimal Local Circuit Ablation} (MnlLCA) \\
{\em Input}: A multi-layer perceptron $M$ of depth $cd$ with $\#n_{tot}$
              neurons and maximum layer width $cw$, connection-value 
              matrices $W_1, W_2, \ldots, W_{cd}$, and bias vector $B$
              and a Boolean input vector $I$ of length $\#n_{in}$. \\
{\em Output}: A minimal subset $N'$ of the $|N|$ neurons
               in $M$ such that $M(I) \neq M'(I)$ for the MLP $M'$ 
	       induced by $N \setminus N'$.

\vspace*{0.1in}

\noindent
{\sc Minimal Global Circuit Ablation} (MnlGCA) \\
{\em Input}: A multi-layer perceptron $M$ of depth $cd$ with $\#n_{tot}$
              neurons and maximum layer width $cw$, connection-value 
              matrices $W_1, W_2, \ldots, W_{cd}$, and neuron bias 
	      vector $B$. \\
{\em Output}: A minimal subset $N'$ of the $|N|$ neurons
               in $M$ such that for the MLP $M'$ induced by $N \setminus 
	       N'$, $M(I) \neq M'(I)$ for every possible Boolean input
	       vector $I$ of length $\#n_{in}$.

\vspace*{0.1in}

\noindent
Given any solution problem {\bf X} above, let \#{\bf X} be the problem that 
returns the number of solution outputs. To assess the complexity of
these counting problems, we will use the following definitions in
\cite[Section 7.3]{GJ79} adapted from those originally given in 
\cite{Val79Enum}.

\begin{definition}
\cite[Page 168]{GJ79}
A counting problem \#{$\Pi$} is in \#P if there is a nondeterministic 
algorithm such that for each input $I$ of $\Pi$, (1) the number of `distinct 
``guesses'' that lead to acceptance of $I$ exactly equals the number 
solutions of $\Pi$ for input $I$ and (2) the length of the longest accepting
computation is bounded by a polynomial in $|I|$.
\end{definition}

\noindent
\#P contains very hard problems, as it is known every class in the
Polynomial Hierarchy (which include $P$ and $NP$ as its lowest members)
Turing reduces to \#P, i.e., $PH \subseteq P^{\#P}$ \cite{Tod91}. We
use the following type of reduction to isolate problems that are
the hardest (\#P-complete) and at least as hard as the hardest
(\#P-hard) in \#P.

\begin{definition}
\cite[Pages 168--169]{GJ79}
Given two solution problems $\Pi$ and $\Pi'$, a {\em (polynomial time)
parsimonious reduction from $\Pi$ to $\Pi'$} is a function $f : I_{\Pi}
\rightarrow I_{\Pi'}$ that can be computed in polynomial time such that
for every $I \in{\Pi}$, the number of solutions of $\Pi$ for input $I$ 
is exactly equal to the number of $\Pi'$ for input $f(I)$.
\end{definition}

\noindent
Reductions are often established to be parsimonious by proving bijections 
between solution-sets for $I$ and $f(I)$, i.e., each solution to $I$ 
corresponds to exactly one solution for $f(I)$ and vice versa.

\section{Results}

\subsection{Results for Minimal Sufficient Circuits}

\begin{theorem}
MnlLSC is polynomial-time solvable.
%
\label{ThmMinLSCPoly}
\end{theorem}

\begin{proof}
Consider the following algorithm:

\begin{verbatim}
      algorithm findMnlLSC(M, I):
   1. C = M
   2. L = the set of all neurons in M
   3. while L is not empty
   4.    randomly select a neuron x in L
   5,    L = L - {x}
   6.    if (C/{x}(I) = M(I) then
   7.       C = C - {x}
   8.       L = the set of all neurons in C 
   9. return C
\end{verbatim}

\noindent
This algorithm essentially derives a minimal local sufficient circuit
by random local search starting with the trivial minimum local sufficient
circuit $C = M$. As at most $|M|$ neurons can be removed from $M$ to
create $C$ and each such removal results in a list $L$ with at most
$|M|$ neurons, the {\sc while} loop in the algorithm executes $O(|M|^2)$
times. As each operation in the algorithm can be done in time polynomial
in $|M|$ and $|I|$, this algorithm runs in polynomial time, giving
the result.
\end{proof}

\begin{theorem}
\#MnlLSC is \#P-complete.
%
\label{ThmMnlLSCsPc}
\end{theorem}
%
\begin{proof}
Consider the reduction from MnlVC to MnlLSC created by modifying the 
reduction
from VC to MLSC given in the proof of Theorem 5 in \cite{War23_MSCR} such
that the bias and input-line weight of input neuron $n_{in}$ are changed
to 0 and 1 to ensure that all possible input vectors (namely, $\{0\}$ and
$\{1\}$) cause $n_{in}$ to output 1. Observe that this modified reduction
runs in time polynomial in the size of the given instance of MnlVC.
We now need to show that this reduction is parsimonious, i.e., this
reduction creates a bijection between the
solution-sets of the given instance of MnlVC and the constructed instance
of MnlLSC.  We prove the two directions of this bijection separately as 
follows:

\begin{description}
\item [$\Rightarrow$]: Let $V' = \{v'_1, v'_2, \ldots, v'_k\} \subseteq V$ 
       be a minimal vertex cover in $G$. Consider the subcircuit $C$ based 
       on neurons $n_{in}$, $n_{out}$, $\{nv'N ~|~ v' \in V'\}$, 
       $\{neA_1, neA_2, \ldots, neA_{|E|}\}$, and
       $\{neN_1, neN_2, \ldots, neN_{|E|}\}$.  
       As shown in the $\Rightarrow$-portion of the proof of correctness
       of the reduction in the proof of Theorem 5 in \cite{War23_MSCR},
       $C$ is behaviorally equivalent to $M$ on $I$.
       As $V'$ is minimal and only vertex NOT neurons can be
       deleted from $M$ to create $C$, $C$ must itself be 
       minimal. Moreover, note that any such set $V'$ in $G$ is associated
       with exactly one set of vertex NOT neurons in (and thus exactly
       one sufficient circuit of) $M$.
\item [$\Leftarrow$]: Let $C$ be a minimal subcircuit of $M$ that is 
       behaviorally equivalent to $M$ on input $I$. As neurons in all five 
       layers in $M$ must be present in $C$ to produce the required output,
       both $n_{in}$ and $n_{out}$ are in $C$. In order for $n_{out}$
       to produce a non-zero output, all $|E|$ edge NOT neurons and all
       $|E|$ AND neurons must also be in $C$, and each of the latter must 
       be connected to at least one of the vertex NOT neurons corresponding
       to their endpoint vertices. Hence, the vertices in $G$ corresponding
       to the vertex NOT neurons in $C$ must form a vertex cover in $G$.
       As $C$ is minimal and only vertex NOT neurons can be
       deleted from $M$ to create $C$, this vertex cover must itself be 
       minimal. Moreover, note that any such set of vertex NOT neurons in
       $M$ is associated with exactly one set of vertices in (and hence
       exactly one vertex cover of) $G$.
\end{description}

\noindent
As \#MnlVC is \#P-complete \cite[Theorem 1(4)]{Val79Enum}, the reduction 
above establishes that \#MnlLSC is \#P-hard.  Membership of \#MnlLSC in 
\#P and hence the result follows from the nondeterministic algorithm for 
\#MnlLSC that, on each computation path, guesses a selection $N'$ of the 
vertex NOT neurons in $M$ and then verifies that the circuit $C$ created 
by deleting $N'$ is minimal and behaviorally equivalent to $M$ on $I$.
\end{proof}

\vspace*{0.1in}

\noindent
Theorems \ref{ThmMinLSCPoly} and \ref{ThmMnlLSCsPc} may at first glance
seem contradictory. However, it is well-known that the complexity of
a solution problem does not dictate the complexity of its associated
counting problem. For instance, SAT and \#SAT are $NP$- and \#P-complete,
respectively, but the problem of finding a perfect matching in a given
bipartite graph is polynomial-time solvable and its associated counting
problem is \#P-complete \cite[Page 169]{GJ79}.

\begin{theorem}
\#MnlGSC is \#P-hard.
%
\label{ThmMnlGSCsPh}
\end{theorem}
%
\begin{proof}
Recall that the parsimonious reduction from MnlVC to MnlLSC in the proof of
Theorem \ref{ThmMnlLSCsPc} creates an instance of MnlLSC whose MLP $M$
has the same output for every possible input vector; hence, this reduction
is also a parsimonious reduction from MnlVC to MnlGSC.
As \#MnlVC is \#P-complete \cite[Theorem 1(4)]{Val79Enum}, this reduction 
establishes that \#MnlGSC is \#P-hard, giving the result.  
\end{proof}

\vspace*{0.1in}

\noindent
Consider \#BMnlLSC and \#BMnlGSC, the versions of \$MnlLSC and \#MnlGSC) in
which one is asked to count the number of minimal local and global 
sufficient circuits of a size $k$ specified as part of the input. These
problems have trivial parsimonious reductions from \#MnlLSC and \#MnlGSC
in which $k$ is the size of the MLP $M$ in the problem instances 
constructed by the reduction and are hence themselves \#P-complete and
\#P-hard.

\subsection{Results for Minimal Necessary Circuits}

\begin{theorem}
\#MnlLCA is \#P-complete.
%
\label{ThmMnlLCAsPc}
\end{theorem}
%
\begin{proof}
Consider the reduction from MnlVC to MnlLCA created by modifying the 
reduction from {\sc Dominating set} to MLCA given in the proof of Theorem 5
in \cite{War24_MCAC} such that the vertex neighbourhood AND and NOT neurons
are re-coded as edge AND and NOT neurons. Observe that this modified 
reduction runs in time polynomial in the size of the given instance of 
MnlVC. We now need to show that this reduction is parsimonious, i.e., this
reduction creates a bijection between the
solution-sets of the given instance of MnlVC and the constructed instance
of MnlLCA.  We prove the two directions of this bijection separately as 
follows:

\begin{description}
\item [$\Rightarrow$]: Let $V' = \{v'_1, v'_2, \ldots, v'_k\} \subseteq V$ 
       be a minimal vertex cover in $G$. Consider the subcircuit $C$ based 
       on neurons $n_{in}$, $n_{out}$, $\{nv' ~|~ v' \in V'\}$, 
       $\{neA_1, neA_2, \ldots, neA_{|E|}\}$, and
       $\{neN_1, neN_2, \ldots, neN_{|E|}\}$.  
       As shown in the $\Rightarrow$-portion of the proof of correctness
       of the reduction in the proof of Theorem 5 in \cite{War23_MSCR}, $C$
       is not behaviorally equivalent to $M$ on $I$. As $V'$ is minimal and
       only input vertex neurons can be deleted from $M$ to create $C$, $C$
       must itself be minimally ablated relative to $M$. Moreover, note that
       any such set $V'$ in $G$ is associated with exactly one set of input
       vertex neurons in (and thus exactly one circuit ablation for) $M$.
\item [$\Leftarrow$]: Let $C$ be a minimally-ablated subcircuit of $M$ 
       such that $C(I) \neq M(I)$. As neurons in all four 
       layers in $M$ must be present in $C$ to produce the required output,
       $n_{out}$ and at least one of the input vertex neurons are in $C$. 
       In order for $n_{out}$ to produce an output, all $|E|$ edge NOT 
       neurons and all $|E|$ AND neurons must also be in $C$, and each of 
       the latter must be connected to at least one of the input vertex 
       neurons corresponding to their endpoint vertices. Hence, the vertices
       in $G$ corresponding to the input vertex neurons in $C$ must form a 
       vertex cover in $G$.  As $C$ is minimally ablated and only input
       vertex neurons can be deleted from $M$ to create $C$, this vertex 
       cover must itself be minimal. Moreover, note that any such set of 
       input vertex neurons in $M$ is associated with exactly one set of 
       vertices in (and hence exactly one vertex cover of) $G$.
\end{description}

\noindent
As \#MnlVC is \#P-complete \cite[Theorem 1(4)]{Val79Enum}, the reduction 
above establishes that \#MnlLCA is \#P-hard.  Membership of \#MnlLCA in 
\#P and hence the result follows from the nondeterministic algorithm for 
\#MnlLSC that, on each computation path, guesses a selection $N'$ of the 
input vertex NOT in $M$ and then verifies that the circuit $C$ created 
by deleting $N'$ is minimal and not behaviorally equivalent to $M$ on $I$.
\end{proof}

\vspace*{0.1in}

\begin{theorem}
\#MnlGCA is \#P-hard.
%
\label{ThmMnlGCAsPh}
\end{theorem}
%
\begin{proof}
Recall that the parsimonious reduction from MnlVC to MnlLCA in the proof of
Theorem \ref{ThmMnlLCAsPc} creates an instance of MnlLCA whose MLP $M$
has the same output for every possible input vector; hence, this reduction
is also a parsimonious reduction from MnlVC to MnlGCA.
As \#MnlVC is \#P-complete \cite[Theorem 1(4)]{Val79Enum}, this reduction 
establishes that \#MnlGCA is \#P-hard, giving the result.  
\end{proof}

\vspace*{0.1in}

\begin{theorem}
\#MnlLNC is \#P-hard.
%
\label{ThmMnlLNCsPh}
\end{theorem}
%
\begin{proof}
Recall that, courtesy of Lemma 2 in \cite{War24_MNC}, for some neuron-subset
$H$ of $M$ and input vector $I$ for $M$, $H$ is a circuit ablation of $M$ 
such that $(M/H)(I) \neq M(I)$ if and only if $H$ is also a necessary 
circuit for $M$ relative to $I$. Hence, every minimal circuit ablation
for $M$ relative t o $I$ is also a minimal necessary circuit for $M$
and vice versa, which means that the parsimonious reduction from MnlVC
to MnlLCA in the proof of Theorem \ref{ThmMnlLCAsPc} is also a 
parsimonious reduction from MnlVC to MnlLNC. The result then follows from 
the \#P-completeness of \#MnlVC \cite[Theorem 1(4)]{Val79Enum}.
\end{proof}

\vspace*{0.1in}

\begin{theorem}
\#MnlGNC is \#P-hard.
%
\label{ThmMnlGNCsPh}
\end{theorem}
%
\begin{proof}
Recall that, courtesy of Lemma 4 in \cite{War24_MNC}, some neuron-subset
$H$ of $M$ is a circuit ablation of $M$ such that $(M/H)(I) \neq M(I)$ 
for every possible input vector $I$ for $M$ if and only if $H$ is also a 
necessary circuit for $M$ relative to every possible input vector $I$ for
$M$. Hence, every minimal global circuit ablation for $M$ is also a minimal
global  necessary circuit for $M$ and vice versa, which means that the 
parsimonious reduction from MnlVC to MnlGCA in the proof of Theorem 
\ref{ThmMnlGCAsPh} is also a parsimonious reduction from MnlVC to MnlGNC.
The result then follows from the \#P-completeness of \#MnlVC 
\cite[Theorem 1(4)]{Val79Enum}.
\end{proof}

\vspace*{0.1in}

\noindent
Consider \#BMnlLNC and \#BMnlGNC, the versions of \$MnlLNC and \#MnlGNC) in
which one is asked to count the number of minimal local and global 
sufficient circuits of a size $k$ specified as part of the input. These
problems have trivial parsimonious reductions from \#MnlLNC and \#MnlGNC
in which $k$ is the size of the MLP $M$ in the problem instances 
constructed by the reduction and are hence themselves \#P-complete and
\#P-hard.


==> tables/table-parameters.tex <==
% \vspace{-15pt}

\begin{wraptable}{l}{\linewidth}
    \caption{Model and circuit parameterizations.}
    \centering
    % \resizebox{200pt}{!}{%
    \small{
    \begin{tabular}{p{0.46\linewidth} | P{0.19\linewidth} P{0.16\linewidth}}
        \toprule
            {\textbf{Parameter}} & \textit{Model (given)} & \textit{Circuit \newline (requested)}\\
            % \cline{2-3}
        \midrule
            \CCG Number of layers (depth) & \CCG $\hat{L}$ & $\hat{l}$\\
            \CCG Maximum layer width & \CCG $\hat{L}_w$ & $\hat{l}_w$\\
            \CCB Total number of units\footnotemark & \CCB $\hat{U} = |\mc{M}| \newline \leq \hat{L} \cdot \hat{L}_w$ & $|\mc{C}|=\hat{u}$\\
            Number of input units & $\hat{U}_I$ & $\hat{u}_I$\\
            Number of output units & $\hat{U}_O$ & $\hat{u}_O$\\
            Maximum weight & $\hat{W}$ & $\hat{w}$\\
            Maximum bias & $\hat{B}$ & $\hat{b}$\\
         \bottomrule
    \end{tabular}
    % }
    }
    \namedlabel{tbl:params}{parameter table}
\end{wraptable}

% \footnotetext{Note the colored parameters bound the input size if bounded (hence vacuously making problems tractable). We avoid this in analyses.}

% \vspace{-10pt}
